TOD: GPU-accelerated Outlier Detection via Tensor Operations

Outlier detection (OD) is a key learning task for finding rare and deviant data samples, with many time-critical applications such as fraud detection and intrusion detection. In this work, we propose TOD, the first tensor-based system for efficient and scalable outlier detection on distributed multi-GPU machines. A key idea behind TOD is decomposing complex OD applications into a small collection of basic tensor algebra operators. This decomposition enables TOD to accelerate OD computations by leveraging recent advances in deep learning infrastructure in both hardware and software. Moreover, to deploy memory-intensive OD applications on modern GPUs with limited on-device memory, we introduce two key techniques. First, provable quantization speeds up OD computations and reduces its memory footprint by automatically performing specific floating-point operations in lower precision while provably guaranteeing no accuracy loss. Second, to exploit the aggregated compute resources and memory capacity of multiple GPUs, we introduce automatic batching, which decomposes OD computations into small batches for both sequential execution on a single GPU and parallel execution on multiple GPUs. TOD supports a diverse set of OD algorithms. Extensive evaluation on 11 real and 3 synthetic OD datasets shows that TOD is on average 10.9x faster than the leading CPU-based OD system PyOD (with a maximum speedup of 38.9x), and can handle much larger datasets than existing GPU-based OD systems. In addition, TOD allows easy integration of new OD operators, enabling fast prototyping of emerging and yet-to-discovered OD algorithms.

==> 09backupintro.tex <==
Outlier detection (OD) is a key machine learning task for identifying data points deviating from a general distribution \cite{aggarwal2015outlier,yu2016survey,liu2021fairness}. OD has numerous real-world applications, including 
% fraud detection \cite{DBLP:conf/www/PanditCWF07}, 
anti-money laundering \cite{DBLP:conf/bigdataconf/Lee0WLATF20}, rare disease detection \cite{pang2021deep}, rumor detection \cite{tam2019anomaly}, and network intrusion detection \cite{lazarevic2003comparative}. Over the years, numerous outlier detection algorithms have been proposed for different types of data, including tabular \cite{aggarwal2015outlier,kingsbury2020elle,li2022ecod,zhao2019lscp}, time-series \cite{boniol2020series2graph,lai2021revisiting,boniol2021sand,cao2019efficient}, graph \cite{aggarwal2011outlier,boniol2020graphan}, etc.
% , tabular OD algorithms are the most common ones \cite{aggarwal2015outlier}.  
% Although many new algorithms have been proposed over the years,
Although there is no shortage of detection algorithms, 
OD applications face challenges in scaling to large datasets, both in terms of execution time and memory consumption. To address these challenges, recent work focuses on both developing distributed OD algorithms on CPUs \cite{lozano2005parallel,otey2006fast,angiulli2010distributed,bhaduri2011algorithms,oku2014parallel,yan2017distributed,toliopoulos2020proud,zhao2021suod} and accelerating certain OD algorithms on GPUs \cite{DBLP:journals/tpds/AngiulliBLS16,DBLP:journals/sigkdd/LealG18}. However, existing GPU-based OD solutions only target specific (families of) OD algorithms with limited ability to generalize. For instance, Angiulli et al. \cite{DBLP:journals/tpds/AngiulliBLS16} showcases an example of using GPUs for distance-based algorithms, while handling linear and probabilistic OD algorithms remain unclear under the proposed solution.

Meanwhile, in the last decade, deep neural networks (DNNs) have revolutionized computer vision, natural language processing, and various other fields~\cite{goodfellow2016deep}, in no small part due to the use of modern hardware accelerators (e.g., GPUs and TPUs) for high-performance tensor algebra operations (matrix multiplication, convolution, etc.)~\cite{lecun20191}. In this paper, we ask: {\em can we leverage advances in DNN systems to optimize the performance and scalability of OD algorithms?}
Notably, achieving this goal requires addressing three key challenges.


\begin{figure}[!t] % [!htp]
\centering
  \vspace{0.1in}
  \includegraphics[width=0.48\textwidth]{figures/overview.pdf}
  \caption{System overview. \system abstracts OD algorithms into small building blocks via the \textit{programming model} for deep optimization, with a set of techniques including \textit{provable quantization}, \textit{automatic batching}, and \textit{multi-GPU support}.}
 \label{fig:overview}
\end{figure}

\begin{enumerate}[leftmargin=*]


\item DNN systems provide a {\em tensor-based} programming interface and represent a DNN model as a combination of tensor algebra operations. Deploying OD applications on existing DNN systems requires effectively decomposing a diverse collection of OD algorithms to tensor operations.

\item DNN systems support a set of techniques to reduce the memory footprint on GPUs, such as quantization for executing operations in low-precision. Despite, applying these techniques to OD algorithms requires additional design given most OD algorithms are unsupervised and lack a way for measuring inaccuracy introduced in memory reduction. 

\item Existing DNN systems cannot directly support large-scale OD computations. Modern DNN systems were designed to iteratively process a small {\em batch} of training samples, even though the entire training dataset can be large. However, many OD applications operate on {\em all} samples, such as computing distances between all sample pairs; they typically do not fit on GPUs with limited memory capacity. How to execute them in batch remain unclear for many OD applications.

\end{enumerate}
In this paper, we present \system, a \underline{t}ensor-based \underline{o}utlier \underline{d}etection system that abstracts OD applications into tensor operations for efficient GPU acceleration.
%%%
A key insight behind \system is leveraging both the software and hardware optimizations in DNN systems to enable performant and scalable OD computations.
To the best of our knowledge, \system is the \textit{first} GPU-based OD system that can support a diversity of OD algorithms.
%comprehensive GPU-based system that supports a large number of diverse OD algorithm for GPU acceleration.
Fig.~\ref{fig:overview} shows an overview of \system, which contains three key components:
\begin{enumerate}[leftmargin=*]
\setlength\itemsep{0.025in}
\item \system uses a novel OD programming model that decomposes a complex OD algorithm into a combination of predefined tensor operations, which can benefit from GPU acceleration (\S \ref{sec:model_abstraction}).
\item \system introduces and applies {\em provable quantization} to accelerate unsupervised OD computations and reduce memory requirements by performing specific floating-point operations in lower precision while provably guaranteeing no accuracy loss (\S \ref{sec:quantization}).
\item To overcome the difficulty of executing OD applications in iterations and the resource limits of a single GPU, {\em automatic batching} and {\em multi-GPU support} further decompose OD computations into small batches, which are executed on multiple GPUs in parallel in a pipeline fashion (\S \ref{sec:batching}).
\end{enumerate}

We compare \system against existing CPU- and GPU-based OD systems on both real-world and synthetic datasets. \system is on average 11.6 times faster than PyOD, a state-of-the-art comprehensive CPU-based OD system~\citep{DBLP:journals/jmlr/ZhaoNL19}, and can process a million samples within an hour while PyOD cannot. Compared to existing GPU-based OD systems, \system can handle much larger datasets, while the GPU baselines run out of GPU memory.
Our evaluation further shows that provable quantization, automatic batching, and multi-GPU support are all critical for performant and scalable OD computations.

%In extensive experiments, we compare \system against a state-of-the-art comprehensive CPU system PyOD \citep{DBLP:journals/jmlr/ZhaoNL19}, and also show the benefits of our proposed acceleration components (provable quantization, automatic batching, multi-GPU support) against GPU baseline. Our main experimental finding is that for the datasets we considered, \system is on average 11.9 times faster than PyOD and can handle a million samples within an hour. Notably, it also handles 10$\times$ larger datasets than the GPU baseline, where the latter faces memory bottleneck (i.e., out-of-memory) with big datasets. 

%In extensive experiments, we compare \system against a state-of-the-art comprehensive CPU system PyOD \citep{DBLP:journals/jmlr/ZhaoNL19}, and also show the benefits of our proposed acceleration components (provable quantization, automatic batching, multi-GPU support) against GPU baseline. Our main experimental finding is that for the datasets we considered, \system is on average 11.9 times faster than PyOD and can handle a million samples within an hour. Notably, it also handles 10$\times$ larger datasets than the GPU baseline, where the latter faces memory bottleneck (i.e., out-of-memory) with big datasets. 




\textbf{Extensibility and integration.}
\system is open-sourced\footnote{Open-sourced Library: \url{https://github.com/yzhao062/pytod}} (see \S \ref{sec:api} for API demonstration), which enables easy development of new OD algorithms by leveraging highly optimized tensor operators. Also, \system provides a unified framework for combining classical OD algorithms and deep learning methods. This combination yields a large number of yet-to-be-discovered OD methods. Thus, we believe that \system also provides a platform that enables rapid research and development of novel OD methods.


==> 10cover.tex <==
\clearpage
\newpage

% \onecolumn
\section*{Cover Letter of the Revision of \system}

In what follows, when we quote the meta-reviewer and reviewers, the quoted text is colored in teal \comments{like this}.

\subsection*{Meta Review}
\comments{Thanks for submitting it to VLDB! All reviewers find this paper interesting. They also identified several opportunities for improvement before recommending Accept for this paper, mainly centered around missing explanations of some critical designs and presentations. The reviewers recommended Revision.}

\noindent We are happy that all reviewers consider \system an interesting work. We have carefully read through all reviews and provided corresponding responses individually. We sincerely appreciate reviewers' constructive and encouraging feedback. We summarize the primary changes in the revision and highlight them in \rv{blue} in the paper:

\begin{itemize}
    \item \textbf{Polished motivation and presentation}: we have updated the abstract and introduction to better motivate the design of \system for scalable and efficient outlier detection. Also, have we revised \S \ref{sec:quantization} and \ref{sec:batching} to provide more details on \textit{provable quantization} and \textit{automatic batching}.
    \item \textbf{Elaboration on limitations, extensibility, and flexibility}: we have included a discussion of TOD’s limitations and extensibility in \S \ref{sec:limitations} and \ref{subsec:implement}, along with new examples of extending \system to build new OD algorithms, such as ECOD and classification model kNN-classifier in Appx. \ref{appx:ecod} and \ref{appx:knn}, respectively. 
    \item \textbf{More real-world datasets}: we have included four additional real-world datasets from a recent anomaly detection benchmark ADBench \cite{han2022adbench}, and updated the evaluation and analysis to include the new results. This addition allows us to evaluate \system on a total of 14 OD datasets, on which \system is on avg. 10.9 times faster than existing OD systems.
    \item \textbf{Additional analysis and ablation studies}: to better understand the advantages of TOD, we provide more detailed time breakdown in Appx. \ref{appx:time_analysis}, a case study on operator fusion in Appx. \ref{appx:fusion_study}, and ablations on provable quantization and automatic batching in Appx. \ref{appx:ablations}.
\end{itemize}

\subsection*{Response to R1}
\comments{\textbf{Q1 \& Q2}. There's a general lack of motivation for OD algorithms. Yes, these are useful, but the paper could be a bit more self-contained and explain what applications would need TOD. Given the extra space available, the paper could be improved by making a stronger case for why OD ops are chosen and by explaining what the limitations of extending the framework beyond OD (limitations and challenges) are.}

\noindent We appreciate the opportunity to provide stronger motivations for building a scalable OD system like TOD. Outlier detection has many critical real-world applications, e.g., fraud detection in credit card transactions, while these time-critical applications often need to process millions of samples within a few seconds/minutes. To address existing OD systems' scalability and efficiency limitations, we build \system to enable these time-critical OD applications to process larger datasets. We appreciate the reviewers’ suggestions and have updated the abstract and the introduction to better motivate the design of \system (e.g., why scalability and efficiency are important to OD applications).

Regarding the extensibility to tasks beyond OD (e.g., classification), we provide an example of using \system for building a k-nearest-neighbor classifier in \S \ref{sec:limitations} and Appx. \ref{appx:knn}. We also note a limitation of building classifiers by TOD---classification tasks often involve optimization using gradient descent, which \system does not specialize in. Thus only calculation-based classifiers can be implemented in \system for now.

In addition, \S \ref{subsec:multigpu} elaborates on the motivation of running OD computation across multiple GPUs in \system. As discussed, OD applications are generally time-critical. Although automatic batching can address the memory limit of a single GPU, deploying OD algorithms across multiple GPUs can largely reduce the run time of these applications, resulting in nearly linear scaling. For instance, the experimental results in \S \ref{subsec:multi_gpu} show that running a kNN detector on 8 GPUs in \system is 7.34$\times$ faster than the single-GPU execution. 

\subsection*{Response to R2}
\comments{\textbf{W1}. There is a lack of discussion about the flexibility and extensibility of the system. 
I am wondering if a researcher wants to design a new outlier detection algorithm, can he/she easily reuse some of the system optimization proposed in this paper? How expressive are the exposed APIs for new algorithm design and implementation? 
R1. Add some necessary discussion about the flexibility and extensibility of the system.}

\noindent We appreciate the comment on discussing TOD’s extensibility and flexibility. \system provides a comprehensive list of BTOs and FOs to support a diverse group of OD algorithms. In the revised paper,  we have added a new section (i.e., \S \ref{subsec:implement}) to discuss the \system's extensibility, including (1) instructions to add new BTOs in \system, (2) developing new OD algorithms in \system, and (3) leveraging \system for classification tasks.

Implementing a new OD algorithm in \system is accessible for an average reader due to the nature of OD algorithms --- they only involve straightforward calculations without complex optimizations. Most OD algorithms depend on only 2-3 BTOs and FOs, with low cognitive complexity. In the revised paper, Appx. \ref{appx:ecod} provides a case study to demonstrate an implementation of the latest ECOD detector (2022) \cite{li2022ecod} in \system. In addition, Appx. \ref{appx:knn} shows another example of using \system to implement a kNN classifier. \\


\noindent \comments{\textbf{W2}. The benchmark datasets do not include real-world large-scale outlier detection tasks.
Second, I notice that the benchmarks are relatively small-scale. In fact, I notice some recent benchmark paper has included more large-scale benchmarks (\url{https://openreview.net/forum?id=foA_SFQ9zo0}), it would make the statement stronger if some more benchmarks could be included. To be more specific, it will be helpful to include some benchmarks with more samples and a lower percentage of anomaly points, e.g., less than 2\%.
Present some additional experiments on tasks with more samples and/or lower percent of anomaly points.}

\noindent Thanks for mentioning our recent ADBench benchmark~\cite{han2022adbench}. Following your advice, we have added four large real-world datasets from ADBench (i.e., celeba, fraud, census, and donors; see Table \ref{table:data}) in the evaluation (see \S \ref{subsec:end_2_end}, and Fig. \ref{fig:full_system_evaluation}). On these new datasets, \system also achieves great performance. For all real-world and synthetic datasets used in the end-to-end evaluation (see \S \ref{subsec:end_2_end}), \system is on avg. 10.9 times faster than existing OD systems.


\subsection*{Response to R3}
\comments{\textbf{D1}. I loved the idea of decomposing the problem into pieces such that each piece can itself be accelerated on GPU. It reminded me of Idreos' Periodic Table of Data Structures [1]. However, many things are not clear.
\begin{enumerate}[label=(\alph*)]
\item Is the list of BTOs complete? Is it possible that there can be another BTO that the authors miss? This should be argued in the paper.
\item Same question for FOs. Is it complete?
\item How do we actually break down an OD algorithm into BTOs and FOs? Figure 3 and Section 4.2 gives an example, but it's quite superficial. It shows one already built tree. I am asking *how* to *build* the tree. Step-by-step, for an average reader.
\item What are the exact details of composing all the OD algorithms in Figure 2? We have known all of them, so we can, at least, build our own intuition on decomposing an OD algorithm into pieces. This can as well be placed in an Appendix or a large technical report. But, this is a must, as otherwise, it is not clear how to combine BTOs and FOs to make an OD algorithm, which is the whole point of the paper. We have to be able to build a clear intuition on how to build an OD algorithm out of BTOs and FOs. Right now, it's at the syntactic level. We need it to be at the semantics level.
\end{enumerate}
}
\noindent \textbf{For (a) and (b)}: The list of BTOs and FOs supported in \system is incomplete (e.g., the current implementation does not support tree-based operators). However, \system still provides a comprehensive list of BTOs and FOs to support a diverse group of OD algorithms, 
and \system can be easily extended to support new OD operators. In the revised paper, \S \ref{sec:limitations} discusses TOD's limitations, and \S \ref{subsec:implement} describes \system's interface to add new OD operators.

\noindent \textbf{For (c) and (d)}: TOD’s programming abstraction is accessible to average readers due to the nature of OD---most OD algorithms only involve straightforward calculation (e.g., density and distance) with 2-3 BTOs and FOs. In the revised paper, Appx. \ref{appx:ecod} and \ref{appx:knn} provide more detailed examples to demonstrate how to implement new OD algorithms in \system.
\\

\noindent \comments{\textbf{D2}. BTOs are on GPU. How about FOs? Do they also run on GPU? If not, do they constitute a bottleneck in the overall execution time. We need an overall execution time breakdown showing what part is accelerated on GPU and what parts are still on CPU. If they are all on GPU, we still need a time breakdown to understand how much time goes to BTO and how much to FO.}

\noindent FOs are decomposed into BTOs and also run on GPUs. To clarify this, Appx. \ref{appx:time_analysis} of the revised paper provides a detailed time breakdown of BTOs and FOs in five OD applications. The results show that GPUs take the most time for heavy lifting computation and thus achieve large performance improvement. Note that Figure~\ref{fig:timebreak} reports the total GPU run time of all BTOs and FOs, since FOs are decomposed into BTOs. \\


\noindent \comments{\textbf{D3}. The provable quantization only applicable 2 ODs out of 8… So, the last sentence just before Section 5.1, “This technique is especially suited for OD operators *as many of them* are mostly ranking and selecting. ”, is simply wrong. Only 2 of 8 are. Let’s remove this sentence. What’s important here is that, for those ODs that are not provable, what are we going to do? What if we run OOM, then? This has to be clearly shown and recognized. Failures are inevitable. But, we have to recognize, quantify and reason about them explicitly. This is actually where the paper gets really interesting.}

\noindent We have removed the “many of them...” sentence in \S \ref{sec:quantization}. We appreciate this opportunity to make the statement more accurate.
Among the eight BTOs and six FOs in the current version of TOD, four operators are generally applicable for provable quantization (i.e., topk, intersect, shared neighbors, and neighbor within range), where we demonstrate the results on two of them in \S \ref{subsec:prov_quant_exp}. Any OD algorithms that depend on these operators (e.g., kNN, LOF, ABOD, and LOCI) can directly benefit from provable quantization. We describe the applicability of provable quantization in \S \ref{subsec:pq_criteria}. 

For OD algorithms where provable quantization is not applicable, \system applies automatic batching to  decompose OD computation into multiple batches, which are equally distributed across GPUs to reduce per-GPU memory requirements. We have added a transition sentence in \S \ref{subsec:pq_criteria} to clarify that other techniques can still apply when provable quantization is disabled. 
Fig. \ref{fig:full_system_evaluation} shows that \system achieves decent performance improvement on HBOS and PCA where provable quantization is not applicable.\\
%Our results on HBOS and PCA (\S \ref{subsec:end_2_end} and Fig. \ref{fig:full_system_evaluation}) show decent performance improvement even when provable quantization is not applicable to these two algorithms. \\

\noindent \comments{\textbf{D4}. Having said that, I don’t understand, though, why only 2 of 8 operators can be used for validation based on Eq. (2). I don’t understand these two requirements in the 2nd paragraph of Section 5.2 to use $\text{Err}(r_q(x))$. Equation (2) can just be used by any operator. In fact, it is actually made for regular +,*,- arithmetic operations. So, to me, anything that produces floating point can be used by (2). I think the authors refer to the case where the accuracy is not compromised. For those cases where the accuracy is not compromised, we can only support 8. This needs to be articulated clearly.}

\noindent All floating-point operations can benefit from direct quantization, while their accuracy is not preserved. Differently, provable quantization performs quantization while provably preserving the final accuracy of the OD algorithm. To clarify this, \S \ref{subsec:pq_criteria} describes the conditions under which provable quantization yields a performance gain (in time/space efficiency).\\

\noindent \comments{\textbf{D5}. Similarly, right before Section 6.1., it says "Using our algorithmic abstraction (see §4), \system provides customized batching solutions for a small number of BTOs with global dependency.". This has to be explained clearly. What are those BTOs? Why for those BTOs are possible and why not for the others? More importantly, what are we going to do for those that we cannot do auto-batch? They will all cause OOM, errors, won't they? In the experimental evaluation, the authors do not report any OOM. Then, the used benchmarks do not cover those BTOs that we cannot do auto-batch. Then, are the used benchmarks inadequate, or are those BTOs not important? If they are not important, why do we even have them in the overall decomposition framework? Right?}

\noindent \system supports automatic batching for \textit{all} BTOs. To achieve this, \system divides BTOs into two categories based on their data dependencies (i.e., whether a sample’s computation depends on other samples and/or requires all features). \system uses different mechanisms to enable batching for operators under different categories. As a result, automatic batching allows \system to execute all BTOs on GPUs without running out of GPU memory. We have revised Fig. \ref{fig:operators} and \S \ref{sec:batching} to clarify that automatic batching applies to all BTOs.\\

\noindent \comments{\textbf{D6}. Section 6.1: Similar problem, when is operation fusion possible and when not..? And, why? This has to be crystal clear, as this is one of the main contributions. Is it possible to get OOMs for those that we cannot fuse? If so, how are we going to solve this problem? Memory is a hard limitation.}

\noindent In the revised paper, \S \ref{subsec:operator_fusion} describes the conditions under which operator fusion is applied in TOD. 
For BTOs and FOs where operator fusion is not applicable, \system automatically batches these operators using simple concatenation (\S \ref{subsec:operator_fusion}) to reduce their memory requirements, thus avoiding OOM issues. 
Appx. \ref{appx:fusion_study} shows a comparison between operator fusion and simple concatenation.\\


\noindent \comments{\textbf{D8}. Is operation fusion only for BTOs, or can FOs also benefit from it?}

\noindent Operator fusion applies to both BTOs and FOs. As an example of fusing FOs, \system fuses k-nearest-neighbors (kNN) and dimensionality reduction (Dim. reduction) by directly conducting kNN on each batch of the compressed data produced by Dim. reduction to avoid data movement. This is clarified in \S \ref{subsec:operator_fusion} of the revised paper.\\


\noindent \comments{\textbf{D9.} Section 6.2: How can we make sure the assigned subtasks are equally distributed? It can easily be skewed, isn’t it? Do you have a cost model telling you how much each subtask will take? If not, how do you do that?}

\noindent The cost of most OD operators only depends on the input tensor size and is independent of the content of the input tensors. By leveraging this property of OD computation, \system can achieve perfectly balanced workload distribution on homogeneous GPUs by equally partitioning input samples across the GPUs. Future work may extend to heterogeneous GPUs. We add these points in \S \ref{subsec:multigpu} and \S \ref{sec:limitations}.\\

\noindent \comments{\textbf{D10}. Section 7.3 and 7.4: How much of the improvement comes from provable quantization and how much from automatic batching… Now, it’s impossible to judge. Both for memory and time.}

\noindent In Appx. \ref{appx:ablations} of the revised paper, we have included an ablation study to evaluate the performance of automatic batching (AB) and provable quantization (PQ) and their combination on both the run time and memory usage. The results show that AB addresses the OOM issue on large datasets, while PQ reduces both the memory consumption and run time. The ablation study also indicates that enabling both techniques leads to the best performance.\\



\noindent \comments{\textbf{D11}. Figure 8: What are the expected lines? Why are they there? And, how do you calculate them? How much is due to quantization and how much auto-batching…? Quantization also helps for memory, doesn’t it?} 
% \todo{It seems we don't answer the last three questions.}

\noindent Thanks for this clarification question. We calculated the expected run time based on the time complexity in Table \ref{table:algorithms}, which may be unclear in the original Fig. \ref{fig:scalability}. In the revised paper, we remove the expected line (the red dotted lines) and only keep the actual run time of each algorithm with regard to an increasing number of samples. We provide an ablation study of provable quantization and automatic batching in Appx. \ref{appx:ablations}, where we observe that both techniques reduce the GPU memory footprint.\\
%The results show that \system has great scalability and roughly follows the expected time complexity. \\ 


\noindent \comments{\textbf{D12}. Section 7.5: What do we lose for provable quantization? If we do non-provable quantization, how much can we get?}

\noindent Provable quantization reduces the memory requirement and execution time of some OD operators while guaranteeing no accuracy loss, while existing (non-provable) quantization techniques directly execute OD operators in low precision without post-verification, resulting in accuracy variation.

In \S~\ref{subsec:prov_quant_exp}, we measure the accuracy variation (e.g., ROC-AUC) by running kNN detector on the fraud, census, and donors datasets in 16-bit precision without post-verification, which leads to -3.48\%, +1.05\%, -4.27\% accuracy variation. These results show the merit of provable quantization over direct quantization. \\

\noindent \comments{\textbf{D13}. Table 4 contradicts with what the authors say in the parag. previous to Case study on runtime breakdown. In the prev. parag. it says 32-bit is slower b/c of post-verification overhead, whereas Table 4 shows that post-verification is negligible...}


\noindent We sincerely appreciate that the reviewer identifies this issue. We double-checked our code and realized that when we measured the run time of 64-bit operations without provable quantization, we mistakenly set its precision in 32-bit. Because of this, 32-bit probable quantization takes more time than 64-bit execution without quantization. By running the experiments with the right setting and correcting Table \ref{table:quantization}, we find that (1) for large datasets, both provable quantization in 16-bit and 32-bit precision are faster than the 64-bit operations without provable quantization for large datasets, and (2) for small datasets, provable quantization does not necessarily improve the run time due to the additional verification and data movement overhead (all settings can finish in 0.1 seconds), while it can still reduce memory requirements. 
We have updated \S \ref{subsec:prov_quant_exp} based on the new results, and sincerely thank you for helping us to improve the paper. \\



\clearpage

==> abstract_submitted.tex <==
Outlier detection (OD) is a key learning task for finding rare and deviant data samples, with many time-critical applications such as fraud detection and intrusion detection. In this work, we propose TOD, the first tensor-based system for efficient and scalable outlier detection on distributed multi-GPU machines. A key idea behind TOD is decomposing complex OD applications into a small collection of basic tensor algebra operators. This decomposition enables TOD to accelerate OD computations by leveraging recent advances in deep learning infrastructure in both hardware and software. Moreover, to deploy memory-intensive OD applications on modern GPUs with limited on-device memory, we introduce two key techniques. First, provable quantization speeds up OD computations and reduces its memory footprint by automatically performing specific floating-point operations in lower precision while provably guaranteeing no accuracy loss. Second, to exploit the aggregated compute resources and memory capacity of multiple GPUs, we introduce automatic batching, which decomposes OD computations into small batches for both sequential execution on a single GPU and parallel execution on multiple GPUs.

TOD supports a diverse set of OD algorithms. Extensive evaluation on 11 real and 3 synthetic OD datasets shows that TOD is on average 10.9x faster than the leading CPU-based OD system PyOD (with a maximum speedup of 38.9x), and can handle much larger datasets than existing GPU-based OD systems. In addition, TOD allows easy integration of new OD operators, enabling fast prototyping of emerging and yet-to-discovered OD algorithms. 
